SLOAM: Semantic Lidar Odometry and Mapping for Forest Inventory

This paper describes an end-to-end pipeline for tree diameter estimation based on semantic segmentation and lidar odometry and mapping. Accurate mapping of this type of environment is challenging since the ground and the trees are surrounded by leaves, thorns and vines, and the sensor typically experiences extreme motion. We propose a semantic feature based pose optimization that simultaneously refines the tree models while estimating the robot pose. The pipeline utilizes a custom virtual reality tool for labeling 3D scans that is used to train a semantic segmentation network. The masked point cloud is used to compute a trellis graph that identifies individual instances and extracts relevant features that are used by the SLAM module. We show that traditional lidar and image based methods fail in the forest environment on both Unmanned Aerial Vehicle (UAV) and hand-carry systems, while our method is more robust, scalable, and automatically generates tree diameter estimations.

==> tex/approach_overview.tex <==
We present an end-to-end pipeline for solving the forest DBH estimation problem. While our approach is specific to our primary forestry problem, the framework and tools we develop are more general to other environments. The pipeline consists: (1) 3D point cloud labeling with virtual reality (VR); (2) range image segmentation with a fully convolutional neural network; (3) landmark instance detection with trellis graphs; (4) semantic lidar odometry; and (5) semantic lidar mapping. We first present the semantic lidar odometry and mapping modules, as they form the core ideas of the work. We then present the first 3 modules which relate to accurate detection of landmarks from individual lidar sensor readings. Finally, we present experimental results of our system in the field.

% We first describe the semantic lidar odometry and mapping algorithms, which represent the last 2 modules in the pipeline and are the core ideas of this work. These modules extends the original ideas in~\cite{zhang2014loam} through the use of features and models based on semantic landmarks. The use of landmarks introduces significant improvements and benefits over local texture-based features. First, the environment-specific landmarks allow us to achieve greater robustness and accuracy since local texture-based features are brittle and unsuitable in natural environments such as forests that feature few planes and edges and feature a lot of noise from surrounding foliage and brush. Second, using only features on the landmarks allow us to immediately remove a large bulk of unnecessary points and retain a sparse set of features, thus speeding up inference speed and is integral in achieving real-time performance. Finally, and most importantly, the use of landmark features allows us to tightly couple the estimation of the sensor state trajectory $\mathcal{X}$ with the estimation of the landmark model parameters in $\mathcal{L}$. Approaches that rely on local texture-based features such as LOAM or Iterative Closest Point (ICP) typically decouple these two problems, and do not use the information contained in the landmarks to aid in the pose estimation. 

% We then present the first 3 modules in the pipeline that describe how to process a raw Lidar sensor reading into a set of landmarks. We utilize a neural network that can be ran in real-time to segment a 2D Lidar range image into landmark classes. In order to easily obtain the labels to train this deep learning framework in a supervised learning fashion, we present a custom virtual reality labeling tool for 3D point cloud labeling. Most applications, such as our DBH estimation problem, do not have standard data sets, but it is critical to easily obtain large, high-quality data sets. Finally, given a lidar segmentation, we present an instance detection algorithm that exploits the structure of the lidar sensor reading to pose the landmark instance detection problem as finding the shortest path through a trellis graph.  

==> tex/instance_detection.tex <==
Since the output of our model only assigns a class to each pixel, to extract the location of each individual landmark a post processing step is required. We can make assumptions about our environment and how the data provided by the lidar is structured making the detection faster and more robust to noise and errors in the segmentation step. The first assumption, that is also made by the methods such as Quickshift ~\ref{qs} and connected component analysis, is that objects have a continuous shape, that is, we should be able to capture the entire structure of the object by grouping nearby points. The second assumption is that the data is gravity aligned, enabling a much more restricted search space and consequently faster instance detection
% this can be achieved by using a sensor that provides gravity orientation such as an IMU, alignment based on the principal component or simply by mounting the sensor in the right orientation with little .
With these assumptions we formalize the instance detection as building with a greedy approach a trellis graph where vertices are connected in slices, defined by different regions of space given by the rows of the organized point cloud provided by the sensor.

% maybe we can have a plot showing the difference between centroid and focus for multiple landmarks
Depending on the perspective the lidar captures an object, its centroid can vary significantly. To get more robustness against view-point changes we compute the focus point $F_v$ of every vertex, that is, the point in the middle of a line defined by the point that is furthest from the centroid and the point furthest from the first, which will be a better estimate of the center of the object.

The instance detection is divided in two alternating steps: First a horizontal search identifies for a row $i$, groups of points from the same class according to the segmented range image that define a vertex of the graph $v_i \in V_g$. This step also uses a lookbehind mechanism to merge two vertices if $euclidean(F_{v_{i-1}}, F_{v_{i}}) < \epsilon$ where $\epsilon$ is a user-defined threshold.
The second step uses a bottom-up approach for matching a sequential pair of rows containing multiple vertices, similarly to the vertex-to-vertex merging mechanism, we create edges between two vertices if their focus point is smaller then a user defined threshold and propagate the instance label of the bottom row to its pair. After the full graph is computed, the output will be a "skeleton" of each instance, that gives a powerful and lightweight representation of the object. A visualization of part of a trellis graph computed with this method is shown in Fig. ~\ref{fig:trellisExample}.


Since the output of our model only assigns a class to each pixel, to extract the location of each individual landmark a post processing step is required. We can make assumptions about our environment and how the data provided by the lidar is structured making the detection faster and more robust to noise and errors in the segmentation step. The first assumption, that is also made by the methods cited, is that objects have a continuous shape, that is, we should be able to capture the entire structure of the object by grouping nearby points. The second assumption is that the data is gravity aligned enabling a much more restricted search space and consequently faster instance detection. With these assumptions we formalize the instance detection as building with a greedy approach a trellis graph where vertices are connected in slices, defined by different regions of space given by the rows of the organized point cloud provided by the sensor.

\begin{figure}[t!]
\centering
\includegraphics[width=\columnwidth]{fig/trellisGraph.png}
\caption{Example of a trellis graph where each node is part of a tree captured by a beam of the lidar, connected to form an instance}
\label{fig:trellisExample}
\end{figure}

==> tex/methodology.tex <==
The semantic localization and mapping problem can be broken down into the following steps: (1) semantic segmentation (2) instance detection (3) landmark description and matching (4) motion estimation and mapping. In figure ~\ref{fig:system} we illustrate the overall pipeline... 

\section{Semantic segmentation}

% more parameters not necessarily mean slower..
The recent classification and segmentation literature has been revolutionized by deep neural network based methods. The biggest drawback of these approaches is the high number of parameters and consequently the difficulty in applying these methods in robot perception tasks that require high frequency outputs. This problem becomes even larger when the sensor being used outputs data of high dimensions such as $360^o$ light detection and ranging sensors (LIDARs).
While some papers have proposed architectures that trade-off accuracy for speed ~\cite{erfnet, mobilenet} the viability of these methods are only becoming a reality now with the advent of specialized hardware and model optimization tools. To enable real-time LIDAR segmentation in the proposed pipeline, we rely on high quality labels generated with a VR labeling tool ~\cite{stevensVRtool} where each scan captured by the LIDAR can be easily manipulated by an human that fits geometric structures to the points that represent objects of interest. The fully convolutional architecture used is a simplified version of ERFNet ~\cite{erfnet} which the operations are optimized for inference with TensorRT ~\cite{trt} gaining up to 3x in speed. Instead of directly segmenting the point cloud, we project the points into a 2D image representation where every pixel is easily mapped back to its original 3D structure, reducing the dimensionality of the problem and making spatial relationships easier to capture by convolution operations one of the drawbacks of this approach is that in some scenarios, this projection will cause some objects to be projected to the same pixel. To reduce this effect, during training and inference we sample the point cloud according to a radius threshold $r$ relative to the origin.
In figure ~\cite{fig:segmentationResults} we illustrate an output in 2D and its projection on the original 3D structure of the environment.

% speed and accuracy go in the results section

\section{Instance detection}

Since the output of our model only assigns a class to each pixel, to extract the location of each individual landmark a post processing step is required. Despite achieving qualitatively good results with approaches such as Quickshift \cite{qshift} and connected components \cite{cc}, we can make more assumptions about our environment and the sensors that makes the detection faster and more robust to noise and errors in the segmentation step. The first assumption, that is also made by the methods cited, is that objects have a continuous shape, that is, we should be able to capture the entire structure of the object by grouping nearby points. The second assumption is that the data is gravity aligned enabling a much more restricted search space and consequently faster instance detection. With these assumptions we formalize the instance detection as building with a greedy approach a trellis graph where vertices are connected in slices, defined by different regions of space given by the rows of the organized point cloud provided by the sensor.

% maybe we can have a plot showing the difference between centroid and focus for multiple landmarks
Depending on the angle the LIDAR captures an object, its centroid can vary significantly. To get more robustness against view-point changes we compute the focus point $F_v$ of every vertex, that is, the point in the middle of a line defined by the point that is furthest from the centroid and the point furthest from the first, which will be a better estimate of the center of the object.

The instance detection is divided in two alternating steps: First a horizontal search identifies for a row $i$, groups of points from the same class according to the segmented range image that define a vertex of the graph $v_i \in V_g$. This step also uses a lookbehind mechanism to merge two vertices if $euclidean(F_{v_{i-1}}, F_{v_{i}}) < \epsilon$ where $\epsilon$ is a user-defined threshold.
The second step uses a bottom-up approach for matching a sequential pair of rows containing multiple vertices, similarly to the vertex-to-vertex merging mechanism, we create edges between two vertices if their focus point is smaller then a user defined threshold and propagate the instance label of the bottom row to its pair. After the full graph is computed, the output will be a "skeleton" of each instance, that gives a powerful and lightweight representation of the object. A visualization of part of a trellis graph computed with this method is shown in figure ~\ref{fig:trellisExample}.

\section{Landmark description and matching}



\section{Motion estimation and mapping}

==> tex/related.tex <==
\begin{figure}[t!]
\includegraphics[width=\columnwidth,trim={2cm 0cm 0cm 0cm},clip]{fig/frontOverview.png}
\caption{Robot platform.}
\label{fig:robot_platform}
\end{figure}

Recently, deploying UAV systems~\cite{Chen2017, Liu2019, Lee2017, 8764006} has been an appealing solution for automated systems and used in a variety of ways including fruit counting~\cite{Chen2017,Liu2019}, disaster management~\cite{Lee2017}, and penstock inspection~\cite{8764006}. Many works of literature~\cite{perez2018architecture, Cui2016, maciel2018extending, Gao2019} focus on autonomous navigation, particularly in cluttered environments~\cite{Gao2019} or GPS-denied areas~\cite{perez2018architecture}.

Focusing on the forestry, many works~\cite{Cui2016, maciel2018extending, Gao2019, Giusti2016, MacielPearson2019, Torresan2017, Puliti2015} employ UAV platforms in foliage environments. Most works~\cite{maciel2018extending, MacielPearson2019, Giusti2016} utilize learning-based approaches to detect the forest trails and enable autonomous navigation of UAVs by following the detected path. However, these works rely on image data for guiding drone’s navigation so there is no mapping module that would provide timber inventory information. Cui et al.~\cite{Cui2016} uses a 2D laser range finder to navigate autonomously in the forest but relying on 2D lidar assumes that vertical direction does not change dramatically. A recent work~\cite{Gao2019} develops a quadrotor platform equipped with a 3D lidar and IMU for navigating in timber environments and building point cloud maps. The forestry applications of UAVs are reviewed in~\cite{Torresan2017, Puliti2015}.

Acquiring timber inventory information is also explored in the literature. Reche et al.~\cite{Reche2011} perform tree modeling from the photograph, and Fritz et al.~\cite{Fritz2013} flies a UAV above the forest and uses photogrammetric point clouds to map the tree stem. Other works~\cite{DeConto2017, liang2016terrestrial} present that tree attributes are estimated by terrestrial laser scanning in forest inventories. The past works rely on photography or TLS that requires time and manpower for timber inventory estimation. The UAVs above forest would not provide accurate forest DBH in case of dense forest.

Our work leverages UAV platforms for measuring timber inventory, particularly diameter at breast height of trees. In this scope, major challenges lie in solving the SLAM problem to accurately estimate the tree attributes. We aim to extend the work of LOAM~\cite{zhang2014loam} for mapping and focus on executing the semantic SLAM~\cite{bowman2017probabilistic} for forestry application. Instead of using positions and classes as semantic measurements~\cite{bowman2017probabilistic}, we utilize a parameterized cylinder as the semantic feature for optimized DBH estimation.

==> tex/segmentation.tex <==
The fully convolutional architecture used is a simplified version of ERFNet ~\cite{romera2017erfnet} where some of the encoder layers are removed. 

Instead of directly operating on the point cloud, the segmentation network takes as input the a 2D range image of size $h x w$ corresponding to the number of beams and azimuth respectively. 

The input is constructed by projecting every 3D point to a pixel according to its position and known parameters of the sensor. This representation makes spatial relationships easier to capture by convolution operations and is more computationally efficient. However, one drawback is that in some scenarios, points that are far away can be projected to nearby pixels and even with different depth values can be challenging to differentiate. To minimize this effect, during training and inference we sample the point cloud $k$ times according to radius range $\gamma$ relative to the sensor. The final mask is given by the sum of all outputs $\sum_{i = 1}^{i=k} f_{seg}(I_{i*\gamma}, w)$ where $I_{i*\gamma}$ is the sampled range image and $f_{seg}$ is the output of the neural network model with weights $w$.

The output of the model is a mask assigning semantic labels for every pixel which are projected back to the corresponding 3D points in the scan. In figure ~\ref{fig:maskVsRaw} we illustrate an output in 2D and its projection on the original 3D structure of the environment.

\begin{figure}[t!]
\centering
\includegraphics[width=0.75\columnwidth]{fig/cloudMaskAndRaw.png}
\caption{Accumulated segmentation (green) against raw point cloud (white).}
\label{fig:maskVsRaw}
\end{figure}


We first segment out points in the point cloud that belong to the ground. We make the basic assumption that the ground is locally planar, but not necessarily globally planar. In a given scan, we first remove points determined to be part of a tree. As a result, we are left with points that belong either to the ground, shrub, or leaves. The key idea is to segmenting out the grounds is that ground appear below all of these other points. However, we can't necessarily just take the lowest points in the cloud, as this approach would fail if the terrain featured a slope or other complicated behavior. As a result, we divide the Lidar cloud into a circular grid determined by the radius and angle of the space around the sensor. Within each grid we retain the lowest $p \%$ of points, where $p$ is a hyperparameter to be tuned. The lower the $p$, the more likely a remaining point is to be a ground, but the less ground features you will have.
